Runtime Verification of Temporal Properties over Out-of-order Data Streams

We present a monitoring approach for verifying systems at runtime. Our approach targets systems whose components communicate with the monitors over unreliable channels, where messages can be delayed or lost. In contrast to prior works, whose property specification languages are limited to propositional temporal logics, our approach handles an extension of the real-time logic MTL with freeze quantifiers for reasoning about data values. We present its underlying theory based on a new three-valued semantics that is well suited to soundly and completely reason online about event streams in the presence of message delay or loss. We also evaluate our approach experimentally. Our prototype implementation processes hundreds of events per second in settings where messages are received out of order.

==> app_proof_mtl.tex <==
\newpage
\section{Soundness and Completeness for the MTL Case}


\newcommand{\tpp}{\mathit{tp}}
\newcommand{\tcp}{\mathit{tc}}
\newcommand{\pos}{\position}
\newcommand{\AP}{\mathit{A}}
\newcommand{\sub}{\mathit{Sub}}
% \newcommand{\intervals}{\mathit{Intv}}

\newcommand{\fPhi}[2]{\Phi_{#1}^{#2}}
\newcommand{\fPsi}[2]{\Psi_{#1}^{#2}}
\newcommand{\fPsip}[2]{\bar\Psi_{#1}^{#2}}

% \newcommand{\deltap}{{{}^\epsilon}\!\delta}
% \newcommand{\deltap}{\bar\delta}
\newcommand{\deltap}{\bar\delta^*}

%% \newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-4.5mu #1\mkern-1.5mu}\mkern 1.5mu}
%% \newcommand{\bAP}{\overbar{\AP}}
\newcommand{\bAP}{\bar{A}}

\newcommand{\by}[1]{\text{\small [by $#1$]}}
\newcommand{\byref}[2]{\text{\small [by (#1): $#2$]}}
\newcommand{\byvar}[2]{\text{\small [by #1: $#2$]}}

\newcommand{\blue}[1]{{\color{blue}#1}}


\subsection{Pseudo-code} 

[TODO: describe; add support for ``complete intervals''.]

Note: Here, \ls{Substitute} also substitutes the atomic propositions
$\tcp^{H,K}$ by the corresponding $\tc^{h,k}$ truth values, if these
values are Boolean.
%
Note: The propositional variables $\bar\alpha^J$ and
$\bar{\bar\alpha}^J$ are treated by the pseudo-code as if they
were~$\alpha^J$. It is only in the proof that we make a distinction
between these propositions.



\begin{listing}[t]
  \centering
  \begin{minipage}[t]{0.15\linewidth}
    \caption{}
    %\caption{The monitor.}
    \label{fig:newmonitor}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.8\linewidth}
\begin{lstlisting}
procedure Monitor($\phi$)
  Init($\phi$)
  loop
    $m$ $\leftarrow$ NewMessage()
    $\tau$, $\sigma$ := Parse($m$)
    NewTimePoint($\tau$, $\phi$)
    foreach $p\in\AP(\phi)$ do
      Propagate($p$, $\set{\tau}$, $\sigma(p)$)

procedure Init($\phi$)
  verdicts := $\emptyset$
  $J_0$ := $[0,\infty)$
  for each $\psi\in \sub(\phi)$ # in a top-down manner
    case $\psi=\neg\alpha$: $\Psi^{\psi,J_0}$ := $\neg \alpha^{J_0}$
    case $\psi=\alpha\lor\beta$: $\Psi^{\psi,J_0}$ := $\alpha^{J_0}\lor \beta^{J_0}$
    case $\psi=\alpha\until_I\beta$: $\Psi^{\psi,J_0}$ := $\tcp^{J_0,J_0} \land \bar\beta^{J_0}\land \bar{\bar\alpha}^{J_0}$
  for each $\alpha$ in Atoms($\phi$) with $\alpha=\true$ do
    Propagate($\alpha$, $J_0$, $\true$)


\end{lstlisting}
  \end{minipage}
\end{listing}
% case $\psi=\freeze{}{x}{\alpha}$: $\Psi^{\psi,J_0}$ := $\alpha^{J_0}$

\begin{listing}[t]
  \centering
  \begin{minipage}[t]{0.15\linewidth}
    \caption{}
    \label{fig:proc1}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.8\linewidth}
\begin{lstlisting}
procedure NewTimePoint($\tau$, $\phi$)
  $J$, new := Split($\tau$)
  marked := $\emptyset$
  for each $\psi\in \sub(\phi)$ # in a top-down manner
    for each $K$ in new do
      case $\psi = \neg\alpha$ then
        $\fPsi{}{\psi,K}$ := Apply($\fPsi{}{\psi,J}$, $[\alpha^J\mapsto \alpha^K]$)
      case $\psi = \alpha\lor\beta$ then
        $\fPsi{}{\psi,K}$ := Apply($\fPsi{}{\psi,J}$, $[\alpha^J\mapsto \alpha^K, \beta^J\mapsto \beta^K]$)
      case $\psi = \alpha\until_I\beta$ then
        $\fPsi{}{\psi,K}$ := Apply($\fPsi{}{\psi,J}$, $[\tcp^{H,J}\mapsto\tcp^{H,K}]_{\tcp^{H,J}\in \AP(\fPsi{}{\psi,J})}$)
    for each $H$ with $\psi^J\in \AP(\fPsi{}{\gamma,H})$ and ($\gamma=\psi\until_I\_$ or $\gamma=\psi\until_I\_$)
      if $(\gamma,H)\notin$ marked then
        marked := marked $\cup$ $\set{(\gamma,H)}$
        $\theta$ := RefinementUntil($\gamma$, $H$, $J$, new)
        $\fPsi{}{\gamma,H}$ := Apply($\fPsi{}{\gamma,H}$, $\theta$)

procedure RefinementUntil($\alpha\until_I\beta$, $H$, $J$, new)
  anchor, continuation $\leftarrow$ $\false$, $\true$
  for $K$ in new with $K\geq H$ do
    if Singleton(K) then cont := $\true$ else $\bar{\bar\alpha}^K$
    anchor := anchor $\lor$ $\bar\beta^K \land \tcp^{K,H} \land \mathsf{cont} \land \mathsf{continuation}$
    continuation $\leftarrow$ continuation $\land$ $\bar\alpha^K$
  return $[\tcp^{J,K}\mapsto\true, \bar\beta^J\mapsto \mathsf{anchor}, \bar\alpha^J\mapsto \mathsf{continuation}, \bar{\bar\alpha}^J\mapsto \true]$
\end{lstlisting}
\end{minipage}
\end{listing}

% the old procedure
%% procedure RefinementUntil($\alpha\until_I\beta$, $K$, $J$, new)
%%   anchor, continuation $\leftarrow$ $\false$, $\true$
%%   for $H$ in new with $H\geq K$ do
%%     if $(K-H)\cap I\not=\emptyset$ then
%%       anchor := anchor $\vee$ $\beta^H$ 
%%       else anchor $\leftarrow$ anchor $\vee$ $\beta^H\wedge\mathsf{continuation}$
%%     continuation $\leftarrow$ continuation $\wedge$ $\alpha^H$
%%   return $[\beta^J\mapsto \mathsf{anchor}, \alpha^J\mapsto \mathsf{continuation}]$

  
\begin{listing}[t]
  \centering
  \begin{minipage}[t]{0.15\linewidth}
    \caption{}
    \label{fig:proc2}
  \end{minipage}
  \quad
  \begin{minipage}[t]{0.8\linewidth}
    \begin{lstlisting}
procedure Apply($\fPsi{}{\psi,J}$, $\theta$)
  $f$ := Substitute($\fPsi{}{\psi,J}$, $\theta$)
  if $f\in\Two$ and CanPropagate($\psi$, $J$, $b$) then
    Propagate($\psi$, $J$, $f$)
  return $f$

procedure Propagate($\psi$, $J$, $b$)
  $\gamma$ := Parent($\psi$)
  if $\gamma$ = nil and Singleton($J$) then
    verdicts := verdicts $\cup$ $\set{(\mathsf{Timestamp}(J),b)}$
  else if CanPropagate($\psi$, $J$, $b$)
    $\theta$ := [$\psi^{J} \mapsto b$]
    foreach $K$ with $\psi^{J}\in \AP(\fPsi{i}{\gamma,K})$
      $\fPsi{i}{\gamma,K}$ := Apply($\fPsi{i}{\gamma,K}$, $\theta$)

procedure CanPropagate($\psi$, $J$, $b$)
  $\gamma$ := Parent($\psi$)    
  case $\gamma$ = nil or $\gamma \neq \_\until_I\_$: return $\true$
  case $\gamma$ = $\_\until_I\psi$: return (Singleton($J$) or not $b$)
  case $\gamma$ = $\psi\until_I\_$: return (Singleton($J$) or $b$)
\end{lstlisting}
\end{minipage}
\end{listing}

%% procedure PropagateTP($i$, $J$)
%%   if Singleton($J$) then
%%     $\theta$ := [$\tpp^{J} \mapsto \true$]
%%     foreach $K$ with $\tpp^{J}\in \AP(\fPsi{i}{\gamma,K})$
%%       ... # repeat the above 3 lines: use a function?

%% procedure PropagateTC($i$, $\psi$, $J$, $K$)
%%   # do the check here or outside?
%%   ...    




\subsection{Proof}


[NOTATION: We denote by $\theta_i(\psi)$ and $\psi\theta_i$ the formula obtained
by instantiating the atomic propositions $p$ in $\psi$ and in
$\pdef(\theta_i)$ by $\theta_i(p)$. We will use the same notation for
other partial valuations.
%
When writing $\theta(x) := \theta'(x)$ we mean that $\theta$ is
undefined on $x$ and has the value $\theta'(x)$ if $\theta'(x)$ if
$\theta'$ is defined on $x$ and otherwise $\theta$ is undefined on
$x$.
%
When writing the definion: it is undefined on all other atomic propositions.

Given two substitutions $\theta$ and $\theta'$ from atomic
propositions to propositional formulas, we write that
$\theta\equiv\theta'$ iff $\pdef(\theta)=\pdef(\theta')$ and $p\theta
\equiv p\theta'$, for any $p\in\pdef(\theta)$.
]




Let $\bar w$ be valid observation sequence and let $\phi$ be the
monitored formula. 
% We assume that $\true$ is not a subformula of $\phi$.
We assume that $\phi$ is not an atomic formula.
%
We let $(J^i_j,\sigma^i_j)$ be the $j$th letter of $w_i$. We
drop the superscript~$i$ if it is clear from the context.
%
Also, given an interval $J$ in $w_i$, we denote by $\hat{J}$ the index
$j\in\pos(w_i)$ such that $J_j = J$, assumming that the iteration~$i$
is clear from the context.


Given an index $i\in\Nat$, an index $j\in\position(w_i)$, and a
non-atomic subformula $\psi$ of $\phi$, we denote by $\Phi_i(\psi,J_j)$
the propositional formula:
\begin{equation*}
  \fPhi{i}{\psi,J_j} := \left\{
    \begin{array}{l@{\quad}l}
      \neg\alpha^{J_j} & \text{if $\psi=\neg\alpha$}
      \\
      \alpha^{J_j}\lor\beta^{J_j} & \text{if $\psi=\alpha\lor\beta$}
      \\
      \bigvee_{k\geq j}\big(\tpp^{J_k} \land \tcp^{J_k,J_j}_\psi \land \beta^{J_k} \land
      \bigwedge_{j\leq h<k}(\tpp^{J_h} \to \alpha^{J_h})
      \big)
      & 
      \text{if $\psi=\alpha\until_I\beta$}
      % \\
      % \qquad\quad \land \bigwedge_{j\leq h<k}(\tpp^{J_h} \to \alpha^{J_h})) \land (\tpp^{J_k} \lor \alpha^{J_k})\big)
      % & 
    \end{array}
    \right.
\end{equation*}
where $\alpha^{K}$, $\tpp^{K}$, and $\tcp^{H,K}_\gamma$ denote atomic
propositions, for each proper subformula~$\alpha$ of $\phi$, each
temporal subformula $\gamma$ of $\phi$, and all intervals $H,K$ of
letters in $w_i$.  We may drop the subscript~$\gamma$ from
$\tcp^{H,K}_\gamma$ when it is clear from the context.
%
We denote by $\AP_i$ the set of these atomic propositions.


We let $\bAP_i$ be the set of atomic propositions obtained from
$\AP_i$ be removing the atomic propositions of the form $\tpp^J$ and
replacing atomic propositions of the form $\beta^J$ and $\alpha^J$
where $\alpha\until_I\beta$ is an subformula of $\phi$ for some $I$,
by the atomic propositions $\bar\beta^J$ and respectively
$\bar\alpha^{J}$ and $\bar{\bar\alpha}^{J}$.
%
Note that $\bAP_i$ represents the set of atomic propositions of the
formulas $\fPsi{i}{\gamma,J}$ from the pseudo-code.


We define the partial valuation~$\theta_i$ of atomic propositions
in $\AP_i$ by
\[\begin{array}{rl@{\quad}l}
  \theta_i(\psi^{J_j}) := & \osem{w_i,j}{\psi} & \text{if $\osem{w_i,j}{\psi}\in\Two$},
  \\
  \theta_i(\tpp^{J_j}) := & \istp_{w_i}(j) & \text{if $\istp_{w_i}(j)\in\Two$},
  \\
  \theta_i(\tcp_{\alpha\until_I\beta}^{J_j,J_k}) := & \tc_{w_i,I}(j,k) & \text{if $\tc_{w_i,I}(j,k)\in\Two$}.
\end{array}\]
We recall that whenever the side condition is not satisifed then
$\theta_i$ is undefined on the corresponding atomic propositions.
%
Also, if $\istp_{w_i}(j)\in\Two$ then $\istp_{w_i}(j)=\true$.
%
%% $\theta_i(\alpha^{J_j})=\osem{w_i,j}{\psi}$ if
%% $\osem{w_i,j}{\alpha}\in\Two$, $\theta_i(\tpp^{J_j})=\true$ if
%% $\istp_{w_i}(j)=\true$,
%% $\tcp_{\alpha\until_I\beta}^{J_j,J_k}=\tc_{w_i,I}(j,k)$ if
%% $\tc_{w_i,I}(j,k)\in\Two$, and otherwise $\theta_i$ is undefined on
%% these atomic propositions.
%
We denote by $\theta_i(\psi)$ and $\psi\theta_i$ the formula obtained
by instantiating the atomic propositions $p$ in $\psi$ and in
$\pdef(\theta_i)$ by $\theta_i(p)$. We will use the same notation for
other partial valuations.
%
It is easy to see that
$$
\theta_i(\fPhi{i}{\psi,J_j}) \equiv \osem{w_i,j}{\psi}
\quad \text{iff} \quad 
\osem{w_i,j}{\psi}\in\Two.
$$
Note also that we have
$\theta_i(\fPhi{i}{\gamma,J})\equiv \theta_i(\gamma^J)$ for any
non-atomic formula $\gamma\neq\phi$.





We state next a lemma that is key to the proof.
%
In order to do that we first introduce some additional notation.

We denote by $\fPsi{i}{\psi,J}$ the value of the variable
$\fPsi{}{\psi,J}$ from the pseudo-code at the end of iteration~$i$.
%
[TODO: intuition for $\deltap$]
%
We also let $\deltap_i$ be the following substitution: 
\begin{align*}
\deltap_i(\bar\beta^J) := &
\left\{
\begin{array}{l@{\quad}l}
\tpp^J\land\beta^J & \text{if $J$ not a singleton and $\fPsi{i}{\beta,J}\notin\Two$}
\\
\tpp^J & \text{if $J$ not a singleton and $\fPsi{i}{\beta,J}=\true$}
\\
\beta^J & \text{if $J$ is a singleton and $\fPsi{i}{\beta,J}\notin\Two$}
\\
\text{undefined} & \text{otherwise}
\end{array}
\right.
\\
\deltap_i(\bar\alpha^J) := &
\left\{
\begin{array}{l@{\quad}l}
\tpp^J\to\alpha^J & \text{if $J$ not a singleton and $\fPsi{i}{\alpha,J}\notin\Two$}
\\
\neg\tpp^J & \text{if $J$ not a singleton and $\fPsi{i}{\alpha,J}=\false$}
\\
\alpha^J & \text{if $J$ is a singleton and $\fPsi{i}{\alpha,J}\notin\Two$}
\\
\text{undefined} & \text{otherwise}
\end{array}
\right.
\\
\deltap_i(\bar{\bar\alpha}^J) := &
\left\{
\begin{array}{l@{\quad}l}
\tpp^J\lor\alpha^J & \text{if $J$ not a singleton and $\fPsi{i}{\alpha,J}\notin\Two$}
\\
\tpp^J & \text{if $J$ not a singleton and $\fPsi{i}{\alpha,J}=\false$}
\\
\alpha^J & \text{if $J$ is a singleton and $\fPsi{i}{\alpha,J}\notin\Two$}
\\
\text{undefined} & \text{otherwise}
\end{array}
\right.
\end{align*}
%
Note that, for instance when $J$ is a singleton and
$\fPsi{i}{\alpha,J}=\true$, there is no need to define
$\deltap_i(\bar\alpha^J)$, because in this case $\bar\alpha^J$ is not
an atomic proposition of $\fPsi{i}{\alpha\until_I\beta,K}$: that
atomic proposition has already been instantiated.







\begin{lemma}\label{lemma:key}
  For any non-atomic subformula $\psi$ of $\phi$, $i\in\Nat$, and
  $j\in\position(w_i)$, we have that
  $\theta_i(\fPhi{i}{\psi,J}) \equiv \deltap_i(\fPsi{i}{\psi,J})$,
  where $J$ is the interval of the $j$th letter of $w_i$.
\end{lemma} 

Observational soundness and completeness follow easily from this
lemma.
%
Indeed, observational soundness follows directly from the lemma and
the above stated properties of $\theta_i$ and $\Phi_i$. Note that
verdicts are only output when $\fPsi{}{\phi,J}\in\Two$ and in that case
we have that $\deltap_i(\fPsi{}{\phi,J}) = \fPsi{}{\phi,J}$.
%
Consider now completeness. Say that $\osem{w_i,j}{\phi}=b\in\Two$ and
$j$ is a time point. Then $\theta_i(\fPhi{i}{\phi,J}) = b$. By the
lemma, we have that $\deltap_i(\fPsi{i}{\phi,J})\in\Two$. If
$\fPsi{i}{\phi,J}$ contains an atomic proposition, then
$\deltap_i(\fPsi{i}{\phi,J})$ would also contain an atomic proposition
(by the definition of $\deltap_i$). Thus it must be the case that
$\fPsi{i}{\phi,J}\in\Two$.  Then there is an iteration $i'\le i$ when
$\fPsi{i'}{\phi,J}$ has been set to a Boolean value. As $J$ is a
singleton, the monitor outputs at that iteration~$i'$ the verdict
$(\tau,b)$ where $J=\set{\tau}$.

\medskip


[TODO: Use $J$ only when we're consider the (arbitrary but fixed)
interval from the lemma. Use some other latter ($H$ or $K$?) when
we're referring to an arbitrary interval.]


We devote the rest of this section to the proof of Lemma~\ref{lemma:key}.
%
We start with an assumption and continue with a series of definitions.

We assume that in the pseudo-code formula rewriting (that is, applying
substitutions) and propagations are separated into two distinct
phases. Note that this can be easily achieved by postponing
propagations, that is, by storing all tuples $(\phi, J, f)$ with
$f\in\Two$ that occur during the execution of \ls{Apply}, and by
performing the corresponding propagations at the end of the
\ls{NewTimePoint} procedure. We choose not to present this two-phase
version of the pseudo-code in order to keep the pseudo-code more
compact.


% the interval~$J'$ in $w_{i-1}$ from which $J$ originates
% (either $J=J'$ or $J$ is one of the three intervals obtained by
% splitting~$J'$).

Let $\mathsf{new}_i$ be the value of \ls{new} at iteration~$i>0$.
[TODO: explain what \ls{new} consists of.]

Given an interval $J\in\mathsf{new}_i$, we let $\zeta^J_i$ be the
substitution computed by the pseudo-code at some iteration~$i>0$
during the formula rewriting phase. Note that there is no formula
rewriting phase at iteration $i=0$. For $i>0$, for instance when
$\alpha$ is such that its parent is $\psi=\neg\alpha$, we have that
$\zeta^J_i(\alpha^{J'})=\alpha^J$ when $J$ is a new interval in $w_i$
obtained by splitting the interval $J'$ in $w_{i-1}$.\footnote{Note
  that in the case of temporal subformulas, this is the composition of
  two substitutions: the unnamed one and the substitution~$\theta$
  computed by \lsf{RefinementUntil}.}
%
% We may drop the superscript~$J$ when it is clear from the context.

% We let $\fPsip{i}{\psi,J}$ be the value of $\fPsi{}{\psi,J}$ at the
% end of the formula rewriting phase of iteration~$i$.
% %
% % For $i=0$, we have $\fPsip{i}{\psi,J} = \zeta^J_i(\fPhi{i}{\psi,J})$. 
% %
% For $i>0$, we have 
% $$
%   \fPsip{i}{\psi,J} = \zeta^J_i(\fPsi{i-1}{\psi,J'}).
% $$


We let $\bar\xi_i$ be the substitution computed by the
pseudo-code at iteration~$i$ during the propagation phase.
%
Formally, $\bar\xi_i$ is a partial valuation over $\bAP_i$ defined as follows:
\begin{align*}
  \bar\xi_i(p^J) :=\ & \quad b\quad \text{if $p\in\AP(\phi)$ and $\sigma^i_{\hat{J}}(p) = b \in \Two$},
  \\
  \bar\xi_i(\gamma^J) :=\ & \quad b\quad \text{if $\gamma$ is non-atomic and $\fPsi{i}{\gamma,J}=b\in\Two$},
  \\
  \bar\xi_i(\bar\beta^J) := &
  \left\{
  \begin{array}{l@{\qquad}l}
    \true  & \text{if $J$ is a singleton and $\fPsi{i}{\beta,J}=\true$},
    \\
    \false & \text{if $\fPsi{i}{\beta,J}=\false$},
  \end{array}\right.
  \\
  \bar\xi_i(\bar\alpha^J) :=
  \bar\xi_i(\bar{\bar\alpha}^J) := &
  \left\{
  \begin{array}{l@{\qquad}l}
    \true  & \text{if $\fPsi{i}{\alpha,J}=\true$},
    \\
    \false & \text{if $J$ is a singleton and $\fPsi{i}{\alpha,J}=\false$},
  \end{array}\right.
  \\
  \bar\xi_i(\tcp_{\alpha\until_I\beta}^{K,J}) := 
  &
  \left\{
    \begin{array}{l@{\qquad}l}
      \true & \text{if $(K-J)\subseteq I$},
      \\
      \false & \text{if $(K-J)\cap I = \emptyset$}.
    \end{array}
  \right.
\end{align*}


% We have that $\fPsi{i}{\psi,J} = \xi_i(\fPsip{i}{\psi,J})$, for any
% $i\in\Nat$, non-atomic subformula~$\psi$ of $\phi$, and interval~$J$
% in $w_i$. 
For any $i>0$, non-atomic subformula~$\psi$ of $\phi$, and
interval~$J$ in $w_i$, we have
\begin{equation}
  \label{eq:Psi}
  \fPsi{i}{\psi,J} := \bar\xi_i(\zeta^J_i(\fPsi{i-1}{\psi,J'})),
\end{equation}
where $J'$ is the interval in $w_{i-1}$ from
which $J$ originates.

We define next the substitution~$\xi_i$ over $\AP_i$ and which is a
variant of $\bar\xi_i$ and which can be seen as the counterpart of
$\theta_i^\Delta$ for the formulas $\fPsi{i}{\gamma,J}$:
\begin{align*}
  \xi_i(p^J) :=\ & \quad b\quad \text{if $p\in\AP(\phi)$ and $\sigma^i_{\hat{J}}(p) = b \in \Two$},
  \\
  \xi_i(\gamma^J) :=\ & \quad b\quad \text{if $\gamma$ is non-atomic and $\fPsi{i}{\gamma,J}=b\in\Two$},
  \\
  \xi_i(\tpp^{J}) :=\ & \true\quad \text{if $J$ is a singleton},
  \\
  \xi_i(\tcp_{\psi}^{K,J}) :=\ & \bar\xi_i(\tcp_{\psi}^{K,J}).
\end{align*}
% $\xi_i(\psi^J)=b$ if $\fPsi{i}{\psi,J}=b\in\Two$,
% $\xi_i(\tpp^{J})=\true$ if $J$ is a singleton, and
% $\xi_i(\tcp_{\alpha\until_I\beta}^{J,K})=\true$ if $(K-J)\subseteq I$,
% and $\xi_i(\tcp_{\alpha\until_I\beta}^{J,K})=\false$ if
% $(K-J)\cap I = \emptyset$.
% % and otherwise $\xi_i$ is undefined on these atomic propositions.




[TODO: intuition] % translation from $\bAP_i$ to $\AP_i$
We also let $\bar\delta_i$ be the following substitution: 
\begin{align*}
\bar\delta_i(\bar\beta^J) & := \tpp^J\land\beta^J,
\\ 
\bar\delta_i(\bar\alpha^J) & := \tpp^J\to\alpha^J,
\\
\bar\delta_i(\bar{\bar\alpha}^J) & := \tpp^J\lor\alpha^J.
\end{align*}
%
Note that we do not have that $\deltap_i = \xi_i \circ
\bar\delta_i$. Indeed, if $\Psi_i^{\beta,J}=\false$ then
$\bar\beta^J\deltap_i=\bar\beta^J$, while
$\bar\beta^J\bar\delta_i\xi_i=\false$.
%
However, as we will prove later, we have that $\deltap_i \circ
\bar\xi_i = \xi_i \circ \bar\delta_i$.

For $i>0$, we define the substitution~$\theta_{i-1,i}$ such that it
behaves as $\theta_{i-1}$, but is however acting on the atomic
propositions of formulas $\fPhi{i}{\gamma,J}$. In other words, in
contrast to $\theta_i$, it does not take into account the new
interpretations received at iteration~$i$. Formally, $\theta_{i-1,i}$
is a partial function over $\AP_i$ defined by
\begin{align*}
  \theta_{i-1,i}(\alpha^{J}) := & \  \theta_{i-1}(\alpha^{J'})
  \\
  \theta_{i-1,i}(\tpp^{J}) := & \  \theta_{i-1}(\tpp^{J'})
  \\
  \theta_{i-1,i}(\tcp^{H,K}) := & \  \theta_{i-1}(\tcp^{H',K'})
\end{align*}
where $J'$, $H'$, and $K'$ are the intervals in $w_{i-1}$ from which
the intervals $J$, $H$, and respectively $K$ originate.


%% $\theta_{i-1,i}(\alpha^{J})=\theta_{i-1}(\alpha^{J})$ if $J$ is the
%% interval of a letter in both $w_{i}$ and $w_{i-1}$ and
%% $\theta_{i-1,i}(\alpha^{J})=\theta_{i-1}(\alpha^{J'})$ if $J$ is the
%% interval of a letter in $w_{i}$ and not in $w_{i-1}$ and $J'$ is the
%% interval of a letter in $w_{i-1}$ with $J\subseteq J'$. By this, we
%% also mean that if $\theta_{i-1}$ is undefined on an atomic
%% proposition, then $\theta_{i-1,i}$ is also undefined on the
%% corresponding atomic proposition.  Furthermore,
%% $\theta_{i-1,i}(\tpp^{J})=\theta_{i-1}(\tpp^{J})$ if $J$ is the
%% interval of a letter in both $w_{i-1}$ and $w_i$, and is undefined
%% otherwise.  Finally, $\theta_{i-1,i}(\tcp^{J,K}) =
%% \theta_{i-1}(\tcp^{J,K})$ if $J$ and $K$ are both the intervals of
%% letters in both $w_{i-1}$ and $w_i$, and is undefined otherwise.


%% We extend $\theta_{i-1}$ such that it is also acting on the
%% atomic propositions of formulas $\fPhi{i}{\psi,J}$. However, in
%% contrast to $\theta_i$, it does not take into account the new
%% interpretations received at iteration~$i$. 
%% %
%% Concretely, on a new atomic proposition~$\alpha^J$ (that is,
%% $\alpha^J\in\AP_i\setminus\AP_{i-1}$, or equivalently where $J$ is the
%% interval of a letter in~$w_i$ and not of a letter in $w_{i-1}$), the
%% value of $\theta_{i-1}$ is the same as the value of (the non-extended)
%% $\theta_{i-1}$ on $\alpha^K$, where $K$ is the interval of a letter in
%% $w_{i-1}$ with $J\subseteq K$. By this, we also mean that if
%% $\theta_{i-1}$ is undefined on an atomic proposition, then $\theta_i'$
%% is also undefined on the corresponding atomic proposition.
%% Furthermore, $\theta_{i-1}(\tpp^{J})$ and $\theta_{i-1}(\tcp^{J,K})$
%% are undefined when $J$ or $K$ are new intervals in~$w_i$.

Finally, we let $\theta_i^\Delta$ be the substitution
defined over $\AP_i$ by
\[\begin{array}{rl@{\quad}l}
\theta_i^\Delta(\alpha^{J}) := & \theta_i(\alpha^{J}) & \text{if $i=0$ or $\theta_{i-1}$ is undefined on $\alpha^{J'}$,}
\\
\theta_i^\Delta(\tpp^J) := & \theta_i(\tpp^J) & \text{if $i=0$ or $\theta_{i-1}$ is undefined on $\tpp^{J'}$,}
\\
\theta_i^\Delta(\tcp^{H,K}) := & \theta_i(\tcp^{H,K}) & \text{if $i=0$ or $\theta_{i-1}$ is undefined on $\tcp^{H',K'}$,}
\end{array}\]
where, when $i>0$, $J'$, $H'$, and $K'$ are the intervals in $w_{i-1}$ from which
the intervals $J$, $H$, and respectively $K$ originate.

Clearly, we have that
\begin{align}
\label{eq:theta}
\theta_i & = \theta_{i-1,i}\, \theta^\Delta_i,\quad \text{for $i>0$},
\\
\label{eq:theta0}
\theta_0 & = \theta^\Delta_0.
\end{align}


To help the reader, we summarize in Table~\ref{tab:substs} all
substitutions used in the proof together with their informal meaning.

\smallskip

\begin{table}[th]
  \label{tab:substs}
  \caption{Summary of substitutions used in the proof.}
  \centering
  \begin{tabular}{|l@{\ }|@{\ }l@{\ }|@{\ }l|}
    \hline
    notation & domain\ & intution  % TODO: here "domain" is used in a large sense
    \\ \hline\hline \rule{0pt}{2.5ex}
    $\theta_i$ & $\AP_i$ & $\gamma^J \mapsto \osem{w_i,\hat{J}}{\gamma}$ if in $\Two$
    \\ \hline \rule{0pt}{2.5ex}
    $\theta_{i-1,i}$ & $\AP_i$ & ''extension'' of $\theta_{i-1}$ from $A_{i-1}$ to $\AP_i$
    \\ \hline \rule{0pt}{2.5ex}
    $\theta_i^\Delta$ & $\AP_i$ & a substitution such that $\theta_i = \theta_{i-1,i}\, \theta_i^\Delta$
    \\ \hline \rule{0pt}{2.5ex}
    $\bar\zeta_i^{J}$ & $\bAP_{i-1}$ & the substitution of the rewriting phase % $\bAP_i\cap \bar{B}_i$
    \\ \hline \rule{0pt}{2.5ex}
    $\zeta_i^J$ & $\AP_{i-1}$ & variant of $\bar\zeta_i^J$ over $\AP_{i-1}$ such that $\bar\zeta^J_i\, \bar\delta_i \equiv \bar\delta_{i-1}\, \zeta^{J}_{i}$ % $\AP_i\cap B_i$
    \\ \hline \rule{0pt}{2.5ex}
    $\bar\xi_i$ & $\bAP_i$ & the substitution of the propagation phase
    \\ \hline \rule{0pt}{2.5ex}
    $\xi_i$ & $\AP_i$ & $\gamma^J \mapsto \fPsi{i}{\gamma,J}$ if in $\Two$
    % \\ \hline \rule{0pt}{2.5ex}
    % $\xi_{i-1,i}$ & $\AP_i$ & ''extension'' of $\xi_{i-1}$ to $\AP_i$
    \\ \hline \rule{0pt}{2.5ex}
    $\bar\delta_i$ & $\bAP_i$ & e.g. $\bar\beta^J\mapsto \tpp^J\land\beta^J$
    \\ \hline \rule{0pt}{2.5ex}
    $\deltap_i$ & $\bAP_i$ & variant of $\bar\delta_i$, taking propagations into account
    % e.g. $\bar\beta^J\mapsto \beta^J$ if $J$ is singleton
    \\ \hline
  \end{tabular}
\end{table}
% \\[2ex]
% where
% \begin{align*}
% \bar{B}_i & = \setx{\bar\beta^{J'}, \bar\alpha^{J'}, \bar{\bar\alpha}^{J'}, \tcp^{H,J'}}{\alpha\until_I\beta\in\sub(\phi), H\geq J'},
% \\
% B_i & = \setx{\beta^{J'}, \alpha^{J'}, \tpp^{J'}, \tcp^{H,J'}}{\alpha\until_I\beta\in\sub(\phi), H \geq J'}.
% \end{align*}
% where $J'$ is the interval that was split at iteration~$i$.




\medskip

Next, we prove Lemma~\ref{lemma:key} by nested induction, the outer
induction being on the iteration~$i$ and the inner induction being a
structural induction on $\psi$.

\emph{Outer base case: $i=0$}. We have a single letter in $w_0$ with the
interval $J=[0,\infty)$. 
%
Let $\fPsip{0}{\psi,J}$ be the value of $\fPsi{}{\psi,J}$ at the point
of execution of the \ls{Init} procedure (thus at iteration~$0$)
between the two \ls{for each} loops, that is, before propagation
of the $\true$~atoms.
%
We thus have that 
\begin{equation}\label{eq:Psi0}
\fPsi{0}{\gamma,J} = \fPsip{0}{\gamma,J}\, \bar\xi_0.
\end{equation}
%
We also have that
\begin{equation}\label{eq:Psi0-Phi0}
\fPsip{0}{\gamma,J}\bar\delta_0 \equiv \fPhi{0}{\gamma,J}.
\end{equation}
%
This is easy to check by inspecting the \ls{Init} procedure. For instance,
for formulas $\gamma=\alpha\until_I\beta$, we have that
$\fPsip{0}{\gamma,J} = \tcp^{J,J} \land \bar\beta^{J} \land
\bar{\bar\alpha}^{J} $ and thus
$$
\fPsip{0}{\gamma,J}\bar\delta_0 
= 
\tcp^{J,J} \land (\tpp^J \land \beta^{J}) \land (\tpp^J\lor \alpha^{J}) 
\equiv 
\tpp^J \land \tcp^{J,J} \land \beta^{J} 
= 
\fPhi{0}{\gamma,J}.
$$

This case then follows from the following sequence of equivalences:
\[
\begin{array}{r@{\quad}l}
%   & \fPhi{i}{\gamma,J}\theta_i
%   & \equiv 
  \blue{\fPsi{0}{\gamma,J}}\, \deltap_0
  \equiv & \byref{\ref{eq:Psi0}}{\fPsi{0}{\gamma,J} = \fPsip{0}{\gamma,J}\, \bar\xi_0}
  \\[0.5ex]
  \fPsip{0}{\gamma,J}\, \blue{\bar\xi_0\, \deltap_0}
  \equiv & \byref{\ref{eq:xi-delta}}{\bar\xi_i\, \deltap_i \equiv \bar\delta_i\, \xi_i}
  \\[0.5ex]
  \blue{\fPsip{0}{\gamma,J}\, \bar\delta_0}\, \xi_0
  \equiv & \byref{\ref{eq:Psi0-Phi0}}{\fPsip{0}{\gamma,J}\, \bar\delta_0 \equiv \fPhi{0}{\gamma,J}}
  \\[0.5ex]
  \fPhi{0}{\gamma,J}\, \blue{\xi_{0}}
  \equiv & \byvar{(\ref{eq:theta0}) and (\ref{eq:xi-theta})}{\xi_{0} \equiv \theta_0}
  \\[0.5ex]
  \fPhi{i}{\gamma,J}\, \theta_{0}
  \ \phantom{\equiv}
\end{array}
\]
We postpone the proof of the not yet justified equivalences (namely
the 2nd and 4th), as similar ones are also used in the inductive case,
and are proved together.





\emph{Outer inductive case: $i>0$}. We assume that the 
equivalence from the lemma statement holds for $i-1$:
\begin{equation}
\label{eq:IH}
\tag{IH}
\fPsi{i-1}{\gamma,J'}\, \deltap_{i-1} \equiv \fPhi{i-1}{\gamma,J'}\, \theta_{i-1}
\end{equation}
where $J'$ is the intervals in~$w_{i-1}$ from which $J$ originates.
%
The inductive case follows from the following sequence of equivalences:
\[
\begin{array}{r@{\quad}l}
%   & \fPhi{i}{\gamma,J}\theta_i
%   & \equiv 
  \blue{\fPsi{i}{\gamma,J}}\, \deltap_i
  \equiv 
  & \byref{\ref{eq:Psi}}{\fPsi{i}{\gamma,J} = \fPsi{i-1}{\gamma,J'}\, \bar\zeta^J_i\, \bar\xi_i}
  \\[0.5ex]
  \fPsi{i-1}{\gamma,J'}\, \bar\zeta^J_i\, \blue{\bar\xi_i\, \deltap_i}
  \equiv 
  & \byref{\ref{eq:xi-delta}}{\bar\xi_i\, \deltap_i \equiv \bar\delta_i\, \xi_i}
  \\[0.5ex]
  \fPsi{i-1}{\gamma,J'}\, \bar\zeta^J_i\, \bar\delta_i\, \blue{\xi_i}
  \equiv 
  & \byref{\ref{eq:xi-idem}}{\xi_i \equiv \xi_{i}\, \xi_{i}}
  \\[0.5ex]
  \fPsi{i-1}{\gamma,J'}\, \blue{\bar\zeta^J_i\, \bar\delta_i}\, \xi_i\, \xi_{i}
  \equiv 
  & \byref{\ref{eq:zeta-delta}}{\bar\zeta^J_i\, \bar\delta_i \equiv \bar\delta_{i-1}\, \zeta^{J}_{i}}
  \\[0.5ex]
  \fPsi{i-1}{\gamma,J'}\, \bar\delta_{i-1}\, \blue{\zeta^{J}_{i}\, \xi_{i}} \, \xi_{i}
  \equiv 
  & \byref{\ref{eq:xi-zeta}}{\zeta^{J}_{i}\, \xi_{i} \equiv \xi_{i-1}\, \zeta^{J}_{i}}
  \\[0.5ex]
  \blue{\fPsi{i-1}{\gamma,J'}\, \bar\delta_{i-1}\, \xi_{i-1}}\, \zeta^{J}_{i}\, \xi_i
  \equiv 
  & \byref{\ref{eq:Psi-xi}}{\fPsi{i-1}{\gamma,J'}\bar\delta_{i-1}\, \xi_{i-1} \equiv \fPsi{i-1}{\gamma,J'}\deltap_{i-1}}
  \\[0.5ex]
  \blue{\fPsi{i-1}{\gamma,J'}\, \deltap_{i-1}}\, \zeta^{J}_{i}\, \xi_i
  \equiv 
  & \byref{\ref{eq:IH}}{\fPsi{i-1}{\gamma,J'}\, \deltap_{i-1} \equiv \fPhi{i-1}{\gamma,J'}\, \theta_{i-1}}
  \\[0.5ex]
  \fPhi{i-1}{\gamma,J'}\, \theta_{i-1}\, \zeta^{J}_{i}\, \blue{\xi_i}
  \equiv 
  & \byref{\ref{eq:xi-theta}}{\xi_i \equiv \theta_i^\Delta}
  \\[0.5ex]
  \fPhi{i-1}{\gamma,J'}\, \blue{\theta_{i-1}\, \zeta^{J}_{i}}\, \theta_i^\Delta
  \equiv 
  & \byref{\ref{eq:zeta-theta}}{\theta_{i-1}\, \zeta^{J}_{i} \equiv \zeta^{J}_{i}\, \theta_{i-1,i}}
  \\[0.5ex]
  \blue{\fPhi{i-1}{\gamma,J'}\, \zeta^{J}_{i}}\, \theta_{i-1,i}\, \theta_i^\Delta
  \equiv 
  & \byref{\ref{eq:Phi-zeta}}{\fPhi{i-1}{\gamma,J'}\, \zeta^{J}_{i} \equiv \fPhi{i}{\gamma,J}}
  \\[0.5ex]
  \fPhi{i}{\gamma,J}\, \blue{\theta_{i-1,i}\, \theta_i^\Delta}
  \equiv 
  & \byref{\ref{eq:theta}}{\theta_{i-1,i}\, \theta_i^\Delta \equiv \theta_{i}}
  \\[0.5ex]
  \fPhi{i}{\gamma,J}\, \theta_{i}
  \ \phantom{\equiv}
\end{array}
\]
where $\zeta^J_i$ is a substitution depending on $\bar\zeta^J_i$.

% As we have that $\fPhi{i}{\gamma,J}\theta_{i-1,i}\theta_{i-1}$, it is
% thus sufficient to show that $\fPhi{i}{\gamma,J}\theta_i =
% \fPhi{i-1}{\gamma,J'}\zeta^{J'}_{i-1}$.

We now complete the proof by proving the not yet justified
equivalences occurring in the above two sequences of equivalences.



\makeatletter
\tagsleft@true
\makeatother

\begin{lemma}
  The following equivalences hold:
    \begin{align}
      \label{eq:xi-idem}
      \xi_i & \equiv \xi_i\, \xi_i
      \\
      \label{eq:xi-theta}
      \xi_i & \equiv \theta_i^\Delta
      \\
      \label{eq:xi-delta}
      \bar\xi_i\, \deltap_i & \equiv \bar\delta_i\, \xi_{i}
      \\
      \label{eq:Psi-xi}
      \fPsi{i}{\gamma,J}\, \deltap_i & \equiv \fPsi{i}{\gamma,J}\bar\delta_i\, \xi_i
    \end{align}
\end{lemma}
\begin{proof} We consider each case in turn.

  \emph{Equivalence~(\ref{eq:xi-idem}).} This case is trivial.
  
  % TODO: This equivalence should be part of the lemma!]
  \emph{Equivalence~(\ref{eq:xi-theta}).} We show that
  $x\xi_i\equiv x\theta_i^\Delta$, for all $x\in\AP_i$.
  % 
  The case when $x$ is one of the atomic propositions $p^J$ with
  $p\in\AP(\phi)$, $\tpp^{J}$, and $\tcp^{H,K}$, follows directly from
  the definitions of~$\xi_i$ and~$\theta_i^\Delta$.
  % 
  Consider now that $x = \gamma^J$ for some non-atomic proper
  subformula~$\gamma$ of $\phi$.
  % 
  We have that $\gamma^J\xi_i$ equals $\fPsi{i}{\gamma,J}$ if
  $\fPsi{i}{\gamma,J}\in\Two$ and equals~$\gamma^J$ otherwise.
   
  Suppose first that $\fPsi{i}{\gamma,J}=b$ for some $b\in\Two$. Then,
  by the inner induction hypothesis, we have that
  $\fPhi{i}{\gamma,J}\theta_i \equiv \fPsi{i}{\gamma,J}\deltap_i
  \equiv b$. As $\fPhi{i}{\gamma,J}\theta_i\equiv \gamma^J\theta_i$,
  we obtain that $\gamma^J\theta_i=b$. 
  % 
  There is then $i'\leq i$ such that
  $\gamma^J\theta_{i'}^\Delta=b$. If $i'=i$ then we're done. If $i'<i$
  then, by the outer induction hypothesis, we obtain that
  $\gamma^{J'}\xi_{i'}=b$, where $J'$ is the interval in $w_{i'}$
  where $J$ originates from. Thus $\fPsi{i'}{\gamma,J'}=b$, from which
  follows that $\fPsi{i}{\gamma,J}=b$ and thus $\gamma^J\xi_i=b$.
  % 
  % TODO: It's a bit unclear what the domain of $\xi_i$ is? Does it
  % include only atomic propositions for the new intervals, or also for
  % the old intervals??
   
  Suppose now that $\fPsi{i}{\gamma,J}\not\in\Two$. Then, using a
  similar reasoning as in the previous case, we obtain that
  $\gamma^J\theta_i\notin\Two$. Thus $\gamma^J\theta_i = \gamma^J$ and
  hence $\gamma^J\theta_i^\Delta = \gamma^J$.

  


  \emph{Equivalence~(\ref{eq:xi-delta}).} This equivalence follows
  directly from the definitions of the four involved substitutions.

  \emph{Equivalence~(\ref{eq:Psi-xi}).} 
  % 
  Let $\fPsip{i}{\gamma,J} := \fPsi{i-1}{\gamma,J'}\bar\zeta^{J}$, for
  $i>0$. From (\ref{eq:Psi}) and~(\ref{eq:Psi0}), we get that, for any
  $i\geq 0$, we need to prove that
  $\fPsip{i}{\gamma,J}\, \bar\xi_i\, \deltap_i \equiv
  \fPsip{i}{\gamma,J}\, \bar\xi_i\, \bar\delta_i\, \xi_i$.
  % 
  This follows directly from equivalence~(\ref{eq:xi-delta}) and the
  equivalence $\bar\xi_i\equiv \bar\xi_i\, \bar\xi_i$.
\end{proof}

\begin{lemma}
  For any~$i>0$ and~$J$ in $\mathsf{new}_i$, there is a
  substitution~$\zeta^{J}_i$ such that for any non-atomic
  formula~$\gamma$ the following equivalences hold:
  \begin{align}
    \label{eq:xi-zeta}
    \zeta^{J}_{i}\, \xi_{i} & \equiv \xi_{i-1}\, \zeta^{J}_{i}
    \\
    \label{eq:zeta-theta}
    \zeta^{J}_{i}\, \theta_{i-1,i} & \equiv \theta_{i-1}\, \zeta^{J}_{i}
    \\
    \label{eq:zeta-delta}
    \bar\zeta^J_i\, \bar\delta_i & \equiv \bar\delta_{i-1}\, \zeta^{J}_{i}
    \\
    \label{eq:Phi-zeta}
    \fPhi{i}{\gamma,J} & \equiv \fPhi{i-1}{\gamma,J'}\, \zeta^{J}_{i}
  \end{align}
  where $J'$ is the interval in $w_{i-1}$ from which $J$ originates.
\end{lemma}
\begin{proof}
  % \emph{Equivalences~(\ref{eq:xi-zeta}), (\ref{eq:zeta-theta}),
  %   (\ref{eq:zeta-delta}) and~(\ref{eq:Phi-zeta}).}
  Let $\psi$ be a proper subformula of $\phi$ and $\gamma$ its parent.
  % 
  For readability, in this proof we drop the index~$i$ from
  $\bar\zeta_i^J$ and $\zeta_i^J$.
  % NOTE: Formally we need to keep it, because the domain changes from
  % one iteration to the other.

  If $\psi$ is a direct subformula of a non-temporal subformula of
  $\phi$, then $\bar\zeta^J(\psi^{J'}) = \psi^J$. In this case we let
  $\zeta^J(\psi^{J'}) := \psi^J$.
  % 
  It is easy to check that the four equivalences hold in this case.
  % 
  % TODO: check say (\ref{eq:xi-zeta}) in one case, say $\neg\alpha$.

  We consider now the case when $\gamma$ is a temporal formula, with
  $\gamma=\alpha\until_I\beta$.
  % 
  % As $\zeta^J_i$ depends on $\bar\zeta^J_i$, which depends on 
  % 
  We first note that for atomic propositions $\bar\beta^{J'}$,
  $\bar\alpha^{J'}$, and $\bar{\bar\alpha}^{J'}$, the
  substitution~$\bar\zeta^J_i$ depends on whether $J$ is $L$, $N$,
  or~$R$, where $\mathsf{new}_i=(L,N,R)$.
  % 
  Thus, we make a case distinction based on the value of~$J$. We only
  consider one case, namely when $J=N$, the other ones being treated
  similarly.
  % 
  In this case we have the following equalities:
  \begin{align*}
    \bar\zeta^N(\bar\beta^{J'}) & = (\bar\beta^N \land \tcp^{N,N}) \lor (\bar\beta^R \land \tcp^{R,N} \land \bar{\bar\alpha}^R \land \bar\alpha^N),
    \\
    \bar\zeta^N(\bar\alpha^{J'}) & = \bar\alpha^N \land \bar\alpha^R,
    \\
    \bar\zeta^N(\bar{\bar\alpha}^{J'}) & = \true, 
    \\
    \bar\zeta^N(\tcp^{{J'},{J'}}) & = \true,
    \\
    \bar\zeta^N(\tcp^{H,{J'}}) & = \tcp^{H,N},\ \text{for $H>{J'}$},
  \end{align*}
  and the substitution $\zeta^N$ is defined as follows
  \begin{align*}
    \zeta^N(\beta^{J'}) & := 
      (\beta^N \land \tpp^{N} \land \tcp^{N,N})\ \lor 
    \\ & \phantom{:=}                 
      (\beta^R \land \tpp^{R} \land \tcp^{R,N} \land 
      (\tpp^R\lor\alpha^R) \land (\tpp^N\to\alpha^N)),
    \\
    \zeta^N(\alpha^{J'}) & := (\tpp^N\to\alpha^N) \land (\tpp^R\to\alpha^R),
    \\
    \zeta^N(\tpp^{{J'}}) & := \true, 
    \\
    \zeta^N(\tcp^{J',J'}) & := \true, 
    \\
    \bar\zeta^N(\tcp^{H,{J'}}) & := \tcp^{H,N},\ \text{for $H>{J'}$}.
  \end{align*}

  By just using the definitions, it is easy to check that the
  equivalences~(\ref{eq:xi-zeta}), (\ref{eq:zeta-theta}), and
  (\ref{eq:zeta-delta}) hold.
  % 
  For instance, we check next that
  $\bar\beta^{J'}\, \bar\zeta^J\, \bar\delta_i \equiv \bar\beta^{J'}\,
  \bar\delta_{i-1}\, \zeta^{J}$: % We have:
  \begin{align*}
    \bar\delta_i(\bar\zeta^N(\bar\beta^{J'})) 
    & = 
      \bar\delta_i\big((\bar\beta^N \land \tcp^{N,N}) \lor
      (\bar\beta^R \land \tcp^{R,N} \land \bar{\bar\alpha}^R \land
      \bar\alpha^N)\big)
    \\ & = 
        ((\tpp^N \land \beta^N) \land \tcp^{N,N})\ \lor
    \\ & \qquad
         ((\tpp^R\land\beta^R) \land \tcp^{R,N} \land (\tpp^R \lor\alpha^R) \land
         (\tpp^N \to\alpha^N))
    \\ & 
        = \zeta^N(\beta^{J'})
        = \zeta^N(\tpp^{J'}\land\beta^{J'})
        = \zeta^N(\bar\delta_{i-1}(\bar\beta^{J'}))
  \end{align*}


  For~(\ref{eq:Phi-zeta}), we check next that
  $\fPhi{i}{\gamma,N} \equiv \fPhi{i-1}{\gamma,J'}\zeta^N$:
  \begin{align*}
    \fPhi{i}{\gamma,N} \equiv\ & 
    \bigvee_{K\geq N}\big(\tpp^{K} \land \tcp^{K,N} \land \beta^{K} \land
    \bigwedge_{N\leq H<K}(\tpp^{H} \to \alpha^{H})
    \big)
    %% 
    % \\ \equiv\ &
    % \bigvee_{K\geq N}\big(\tpp^{K} \land \tcp^{K,N} \land \beta^{K} \land
    % (\tpp^{K} \lor \alpha^{K}) \land
    % \bigwedge_{N\leq H<K}(\tpp^{H} \to \alpha^{H})
    % \big)
    %% 
    \\ \equiv\ & 
    \big(\tpp^{N} \land \tcp^{N,N} \land \beta^{N} \big)
    \lor
    \\ & 
    \big(\tpp^{R} \land \tcp^{R,N} \land \beta^{R} \land (\tpp^{R} \lor \alpha^{R})
    \land (\tpp^{N} \to \alpha^{N}) \big) \lor
    \\ 
    & \bigvee_{K>R}\big(\tpp^{K} \land \tcp^{K,N} \land \beta^{K} \land
    \\ & \hspace*{5em}
    \land (\tpp^{N} \to \alpha^{N}) \land (\tpp^{R} \to \alpha^{R})
    \land \bigwedge_{R<H<K}(\tpp^{H} \to \alpha^{H})
    \big)
    %% 
    \\
    \equiv\ &
    \zeta^N\Big(\big(\tpp^{J} \land \tcp^{J,J} \land \beta^{J}\big) \lor
    \\ & \quad
    \bigvee_{K>J}\big(\tpp^{K} \land \tcp^{K,J} \land \beta^{K} 
    \land (\tpp^{J} \to \alpha^{J}) \land \bigwedge_{J<H<K}(\tpp^{H} \to \alpha^{H})
    \big)\Big)
    %% 
    \\
    \equiv\ & \zeta^N(\fPhi{i-1}{\gamma,J})
  \end{align*}

  % We perform a case distinction on the structure of $\psi$.
  
  % Case $\psi\in\AP(\phi)$.
  
  % Case $\psi=\neg\alpha$.

  % Case $\psi=\alpha\lor\beta$. 
  
  % Case $\psi=\alpha\until_I\beta$.


  % Consider now formulas of the form $\psi=\alpha\until_I\beta$.
  % % 
  % We have four cases to consider:
  % \begin{itemize}
  % \item $J$ is a new interval;
  % \item $\theta_{i-1}(\psi,J)$ contains an atomic proposition $\beta^K$ where $K$ is a new interval;
  % \item $\theta_{i-1}(\psi,J)$ contains an atomic proposition $\alpha^K$ where $K$ is a new interval;
  % \item neither of the above: trivial case, as there are no almost changes...
  % \end{itemize}
\end{proof}

% \begin{align*}
%   \bar\zeta^N(\fPhi{i-1}{\psi,J}) \equiv\ &
%   \bar\zeta^N\Big(\big(\tpp^{J} \land \tcp^{J,J} \land \beta^{J}\big) \lor
%   \\ & 
%   \quad\bigvee_{K>J}\big(\tpp^{K} \land \tcp^{K,J} \land \beta^{K} 
%   \land (\tpp^{J} \to \alpha^{J}) \land \bigwedge_{J<H<K}(\tpp^{H} \to \alpha^{H})
%   \big)\Big)
%   \\
%   \equiv\ &
%   \big(((\beta^N \land \tpp^{N} \land \tcp^{N,N}) \lor (\beta^R \land \tpp^{R} \land \tcp^{R,N} \land
%             (\tpp^R\lor\alpha^R) \land (\tpp^N\to\alpha^N)))\big) \lor
%   \\ & 
%   \bigvee_{K>J}\big(\tpp^{K} \land \tcp^{K,N} \land \beta^{K} \land
%   \\ & \hspace*{5em} 
%   \land (\tpp^{N} \to \alpha^{N}) \land (\tpp^{R} \to \alpha^{R}) \land 
%   \bigwedge_{J<H<K}(\tpp^{H} \to \alpha^{H})
%   \big)
% \end{align*}





%% \bigskip
%% \bigskip

%% Used symbols:
%% \begin{itemize}
%% \item formulas: $\alpha, \beta, \gamma, \phi, \psi$
%% \item interpretations: $\sigma$
%% \item register valuations: $\rho$
%% \item valuations (of variables): $\nu$, $\mu$, $\eta$
%% \item valuations (of atomic propositions): $\theta$, $\zeta$, $\xi$, $\delta$
%% \end{itemize}






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

